On the Laplacian spread of digraphs

In this article, we extend the notion of the Laplacian spread to simple directed graphs (digraphs) using the restricted numerical range. First, we provide Laplacian spread values for several families of digraphs. Then, we prove sharp upper bounds on the Laplacian spread for all polygonal and balanced digraphs. In particular, we show that the validity of the Laplacian spread bound for balanced digraphs is equivalent to the Laplacian spread conjecture for simple undirected graphs, which was conjectured in 2011 and proven in 2021. Moreover, we prove an equivalent statement for weighted balanced digraphs with weights between $0$ and $1$. Finally, we state several open conjectures that are motivated by empirical data.

==> shared.tex <==
% SIAM Shared Information Template
% This is information that is shared between the main document and any
% supplement. If no supplement is required, then this information can
% be included directly in the main document.


% Packages and macros go here
\usepackage{lipsum}
\usepackage{amsfonts}
\usepackage{graphicx}
\usepackage{enumerate}
\usepackage{epstopdf}
\usepackage{microtype}
\usepackage{algorithmic}
%\usepackage{pgfplots}
%\pgfplotsset{compat=1.18}
%\ifpdf
%  \DeclareGraphicsExtensions{.eps,.pdf,.png,.jpg}
%\else
%  \DeclareGraphicsExtensions{.eps}
%\fi

% Add a serial/Oxford comma by default.
\newcommand{\creflastconjunction}{, and~}

% Used for creating new theorem and remark environments
\newsiamremark{remark}{Remark}
\newsiamremark{hypothesis}{Hypothesis}
\crefname{hypothesis}{Hypothesis}{Hypotheses}
\newsiamthm{conjecture}{Conjecture}

% Sets running headers as well as PDF title and authors
%\headers{Laplacian Spread for Digraphs}{W.~Barrett, T.~R.~Cameron, E.~Evans, H.~T.~Hall, and M.~Kempton}

% Title. If the supplement option is on, then "Supplementary Material"
% is automatically inserted before the title.
\title{On the Laplacian spread of digraphs\thanks{This work was supported by the AMS-Simons Travel Grants, which are administered by the American Mathematical Society with support from the Simons Foundation.}}

% Authors: full names plus addresses
\author{Wayne Barrett\thanks{Department of Mathematics, Brigham Young University, Provo, UT (\email{wb@mathematics.byu.edu}, \email{ejevans@math.byu.edu}, \email{mkempton@mathematics.byu.edu}).}
\and Thomas R. Cameron\thanks{Department of Mathematics, Penn State Behrend, Erie, PA 
  (\email{trc5475@psu.edu}).}
\and Emily Evans\footnotemark[2]
\and H.~Tracy Hall\thanks{Hall Labs LLC, Provo, UT 
  (\email{H.Tracy@gmail.com}).}
\and Mark Kempton\footnotemark[2]}

\usepackage{amsopn}
% join commands
\makeatletter
\newcommand{\oset}[3][0ex]{%
 \mathbin{\mathop{#3}\limits^{%
  \vbox to#1{\kern-0.7\ex@
   \hbox{$\scriptstyle#2$}\vss}}}}
\makeatother
\newcommand{\djoin}{\oset{\rightarrow}{\vee}}
\newcommand{\bdjoin}{\oset{\leftrightarrow}{\vee}}
% other commands
\usepackage{mathtools}
\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}
\newcommand*\comp[1]{\overline{#1}}
\newcommand{\iu}{{i\mkern1mu}}
\newcommand\abs[1]{\left|#1\right|}
\newcommand\norm[1]{\left\Vert#1\right\Vert}
\newcommand\re[1]{\operatorname{Re}\mathclose{\left(#1\right)}}
\newcommand\diag[1]{\operatorname{diag}\mathclose{\left(#1\right)}}
\newcommand\conv[1]{\operatorname{conv}\mathclose{\left(#1\right)}}
\newcommand\spn[1]{\operatorname{span}\mathclose{\left(#1\right)}}
\renewcommand\dim[1]{\operatorname{dim}\mathclose{\left(#1\right)}}
\renewcommand\det[1]{\operatorname{det}\mathclose{\left(#1\right)}}
\newcommand\tr[1]{\operatorname{tr}\mathclose{\left(#1\right)}}
\renewcommand\sp[1]{\operatorname{sp}\mathclose{\left(#1\right)}}

%%% Local Variables: 
%%% mode:latex
%%% TeX-master: "ex_article"
%%% End: 

